Diffusion Models for Reinforcement Learning: A Survey

Diffusion models surpass previous generative models in sample quality and training stability. Recent works have shown the advantages of diffusion models in improving reinforcement learning (RL) solutions. This survey aims to provide an overview of this emerging field and hopes to inspire new avenues of research. First, we examine several challenges encountered by RL algorithms. Then, we present a taxonomy of existing methods based on the roles of diffusion models in RL and explore how the preceding challenges are addressed. We further outline successful applications of diffusion models in various RL-related tasks. Finally, we conclude the survey and offer insights into future research directions. We are actively maintaining a GitHub repository for papers and other related resources in utilizing diffusion models in RL: https://github.com/apexrl/Diff4RLSurvey.

==> papers/7-limitation.tex <==
\section{Limitations and Remarks}
\label{sec:limitation}
% \zhengbang{intro}
In this section, we list three limitations when applying diffusion models in RL, and include remarks on comparing diffusion-based generative modeling in RL to transformer-based autoregressive approaches.

\paragraph{Application in online RL.}
Though diffusion models have contributed to offline RL from various perspectives, the dynamic and evolving nature of online RL introduces a significant challenge, as the data distribution sampled by the current policy can change over time. The primary concern is that effectively adapting diffusion models to changing data distributions requires a substantial amount of new data~\cite{lu2023synthetic}. These models are typically trained on fixed datasets, and incorporating enough data to ensure they can generalize and remain effective in dynamic real-world scenarios is a resource-intensive task. Balancing the need for adaptability with the requirement for extensive data is the primary consideration when applying diffusion models in online RL. It is promising to solve this dilemma with more lightweight diffusion models which can keep consistency as the data distribution changes during online interactions.
% \zhengbang{Extend this paragraph}

\paragraph{Iterative sampling cost.}
The unique stepwise denoising mechanism of diffusion models makes the sampling procedure need to infer the trained model multiple times, significantly increasing the sampling cost. Although we can perform sampling acceleration techniques such as DDIM or DPM-Solver, the expensive inference cost limits the model to conduct high-frequency output in online interactions with virtual environments and real-world continuous control scenarios. The problem becomes more severe in those methods that generate a long trajectory but only take the first state or action for execution, such as Diffuser \cite{Janner2022PlanningWD} or Decision Diffuser \cite{decision_diffuser}. 
% Firstly, these models often suffer from extended sampling times, which can be particularly problematic in real-time, online environments where decisions must be made swiftly. 
\citet{chen2023boosting} incorporate the recently proposed Consistency Model \cite{song2023consistency} to enable sampling with one or two diffusion steps, and the performances are comparable to that of DDPM or DDIM with 50 steps.

% \paragraph{Discrete state spaces.}
% Although diffusion models have been verified effective in both continuous and discrete state spaces \cite{sohl2015deep,ho2020denoising,unleash,Gu2021VectorQD}, the works about diffusion models in RL are still limited to continuous spaces. However, there are many RL problems equipped in discrete state space, and how diffusion models perform on such tasks still needs to be explored.

\paragraph{Variance in stochastic sampling.}
In traditional RL algorithms, a continuous control policy is represented by a state-conditioned Gaussian~\cite{haarnoja2018soft,schulman2017proximal}. We can take its mean as action when deterministic execution is required.
However, such deterministic policy is not possible when using diffusion models as the policy class. The randomness of diffusion sampling comes from both initial noise and per-step stochastic denoising. Although per-step stochasticity can be avoided if sampling with ODE-based methods like DDIM, the randomness in initial noisy samples remains inevitable. 
The high-variance policies can have a negative impact in environments with high accuracy or safety requirements.
% However, with diffusion models, we can only draw random samples from the fixed Gaussian white noise, which means we cannot obtain deterministic and consistent results as the denoising procedure is not interpretable and controllable, making the sampling process noisy and high-variance. 
Existing works in RL rarely discuss this limitation, and sampling methods with reduced variances are expected.
% and sampling methods for high-probabilistic action/trajectory are expected.

\paragraph{Comparison to transformer-based methods.}
The idea of using diffusion models commonly abstracts offline RL as a conditional generative modeling problem, differing from traditional RL approaches, which need value function approximations or policy gradient calculation. This supervised learning paradigm is similar to Decision Transformer (DT)~\cite{chen2021decision}, a sequential modeling framework for RL tasks with transformer architecture. The essence of both approaches is to take advantage of the high expressiveness model, where diffusion models enjoy a strong distribution fitting ability to produce multi-modal, diverse, and accurate outputs, and transformers are adept in long-horizon sequence modeling and time correlation understanding. Qualitatively, this difference in expertise makes the diffusion-based approach more suitable for learning complex multi-modal tasks, and Transformer-based approaches~\cite{meng2021offline,wen2022multi} are more preferred in correlated sequence modeling in time or agent (in multi-agent tasks) dimension.

